Attn-GS: Attention-Guided Context Compression for Efficient Personalized LLMs

Personalizing large language models (LLMs) to individual users requires incorporating extensive interaction histories and profiles, but input token constraints make this impractical due to high inference latency and API costs. Existing approaches rely on heuristic methods such as selecting recent interactions or prompting summarization models to compress user profiles. However, these methods treat context as a monolithic whole and fail to consider how LLMs internally process and prioritize different profile components. We investigate whether LLMs' attention patterns can effectively identify important personalization signals for intelligent context compression. Through preliminary studies on representative personalization tasks, we discover that (a) LLMs' attention patterns naturally reveal important signals, and (b) fine-tuning enhances LLMs' ability to distinguish between relevant and irrelevant information. Based on these insights, we propose Attn-GS, an attention-guided context compression framework that leverages attention feedback from a marking model to mark important personalization sentences, then guides a compression model to generate task-relevant, high-quality compressed user contexts. Extensive experiments demonstrate that Attn-GS significantly outperforms various baselines across different tasks, token limits, and settings, achieving performance close to using full context while reducing token usage by 50 times.

==> Sections/Experiment3.tex <==

\section{Can we extract private data from structured-language RAG?}
\label{Ex3}





==> Sections/Experiment4.tex <==


\section{Exploration on Multi-task fine-tuned model Memorization Behavior}
\label{Ex4}

Beyond fine-tuning on a single task, multi-task fine-tuning has been also widely utilized, like \citep{longpre2023flan} \citep{wei2021finetuned}\citep{ouyang2022training} \cite{chung2022scaling}. Multi-task fine-tuning typically leverages a pre-trained language model and continues training across several downstream tasks at a time. Multi-task fine-tuning is a promising approach to enhance the capabilities and generalizability of pre-trained language models for diverse downstream applications. In this section, we investigate the effects of multi-task fine-tuning on model memorization.


\textbf{Observation 1:} \textit{Task disparity still exists in the multi-task fine-tuned model. }
We first examine the memorization behavior of FLAN-T5~\cite{chung2022scaling}, an enhanced version of T5 that has been fine-tuned on over 1,000 additional tasks beyond the original T5 model. We select several popular tasks and datasets that were utilized to fine-tune FLAN-T5 and examine the memorization behavior of FLAN-T5. The results are presented in Table \ref{tab: flan t5}.  On the one hand, similar to single-task fine-tuning, multi-task fine-tuning also presents memorization effects and demonstrates similar task disparity. For instance, we can see the memorization of summarization is obviously higher than other tasks like classification and reading comprehension. 

\textbf{Observation 2:} \textit{Multi-task fine-tuned model prohibit lower memorization ratio compared with single-task fine-tuned model, suggesting its potential to mitigate memorization}
The memorization ratio for high-memorization tasks is substantially lower than that of single-task fine-tuned models. For example, the memorization ratio of summarization 
 (2.96\% on multi\_news and 0.92\% on CNN\_Daily ) in multi-task fine-tuning is much lower compared to that of single-task fine-tuning shown in Table~\ref{tab:self finetune} (22.33\% on Multi\_news)  and Table~\ref{tab:Open_Sourced finetune} (20.7\% on CNN\_Daily). This observation suggests that multi-task fine-tuning has the potential to mitigate the memorization of high-memorization tasks.
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.44\textwidth]{pic/multi_vs_single.pdf}
  \caption{Memorization Comparison of Fine-tuned T5, T5-base, and FLAN-T5 in Summarization on Multi\_News}
  \vspace{-0.3cm}
  \label{fig:multi_vs_single}
\end{figure}



\begin{table*}[]
\centering
\caption{Memorization of FLAN\_T5}
\label{tab: flan t5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|ccccc}
\toprule
Task & Sub\_task & Dataset & Total & Verbatim  & Idea  & \begin{tabular}[c]{@{}c@{}}Paraphrase\\ ($P<0.5$)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Paraphrase\\ ($P>0.5$)\end{tabular} \\ \midrule
\multirow{3}{*}{Summarization} & \multirow{3}{*}{Summarization} & Multi\_news & 2.96\% & 0.73\% & 0.42\% & 0.51\% & 1.81\% \\ 
& & CNN\_Daily & 0.92\% & 0.01\% & 0.16\% & 0.10\% & 0.75\% \\ 
& & Xsum & 0.46\% & 0.01\% & 0.04\% & 0.08\% & 0.41\% \\ \midrule

\multirow{5}{*}{\makecell{ Reading\\Comprehension}} & \multirow{2}{*}{Extractive} & SQuAD\_v2 & 0.06\% & 0.03\% & 0.00\% & 0.00\% & 0.03\% \\ 
& & adversarial\_qa & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ \cmidrule{2-8}

& Abstractive & duorc\_SelfRC & 0.02\% & 0.00\% & 0.00\% & 0.00\% & 0.02\% \\ 
& & duorc\_ParaRC & 0.09\% & 0.00\% & 0.05\% & 0.00\% & 0.04\% \\ \cmidrule{2-8}

& Multiple Choice & boolq & 0.13\% & 0.00\% & 0.02\% & 0.04\% & 0.11\% \\ \midrule

\multirow{2}{*}{Classification} & \multirow{2}{*}{Classification} & AG\_news & 0.03\% & 0.01\% & 0.00\% & 0.01\% & 0.02\% \\ 
& & dbpedia\_14 & 0.03\% & 0.00\% & 0.01\% & 0.01\% & 0.02\% \\ \midrule

\multirow{2}{*}{Translation} & \multirow{2}{*}{Translation} & WMT\_14 & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ 
& & WMT\_16 & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ \midrule

\multirow{2}{*}{NLI} & \multirow{2}{*}{NLI} & super\_glue/cb & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ 
& & super\_glue/wsc & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ \bottomrule
\end{tabular}
}
\end{table*}


To further investigate the impact of multi-task fine-tuning on memorization of high-memorization tasks, we compare the memorization behavior of T5-base (Pre-trained), fine-tuned T5 (single-task fine-tuning), and FLAN-T5 (multi-task fine-tuning) as shown in Figure~\ref{fig:multi_vs_single}. Note that we choose summarization as the high-memorization task and test on the Multi\_News dataset in this study. The high memorization ratio of T5-base (11.03\%) suggests the overlap between the fine-tuning dataset and the pre-training dataset. Notably, the memorization ratio is increased markedly after single-task fine-tuning (22.23\%) compared to T5-base (11.03\%), indicating the single-task fine-tuning process causes the model to memorize more of the training data. On the other hand, the memorization ratio of the multi-task fine-tuned FLAN-T5 (2.96\%) is substantially lower than that of T5-base (11.03\%) and fine-tuned T5 (22.23\%). In particular, the memorization ratio of FLAN-T5 is approximately 5 times lower than T5-base and 10 times lower than fine-tuned T5. These observations further validate that multi-task fine-tuning has the potential to mitigate memorization of high-memorization tasks. A plausible explanation for this observation is the enhanced generalization capability of the model in a multi-task setting. Exposure to a broader array of tasks and data appears to facilitate this improved generalization.  Consequently, the model’s ability to execute tasks is not solely dependent on memorization but also on its refined generalization skills. 

 





